Applications in CityLearn Gym Environment for Multi-Objective Control Benchmarking in Grid-Interactive Buildings and Districts

It is challenging to coordinate multiple distributed energy resources in a single or multiple buildings to ensure efficient and flexible operation. Advanced control algorithms such as model predictive control and reinforcement learning control provide solutions to this problem by effectively managing a distribution of distributed energy resource control tasks while adapting to unique building characteristics, and cooperating towards improving multi-objective key performance indicator. Yet, a research gap for advanced control adoption is the ability to benchmark algorithm performance. CityLearn addresses this gap an open-source Gym environment for the easy implementation and benchmarking of simple rule-based control and advanced algorithms that has an advantage of modeling simplicity, multi-agent control, district-level objectives, and control resiliency assessment. Here we demonstrate the functionalities of CityLearn using 17 different building control problems that have varying complexity with respect to the number of controllable distributed energy resources in buildings, the simplicity of the control algorithm, the control objective, and district size.

==> content/background.tex <==
\section{Background} \label{sec:background}
\subsection{Reinforcement Learning}
\Gls{rl} can be formalized as an \gls{mdp}~\cite{richard_s_sutton_and_andrew_g_barto_reinforcement_2018}. An \gls{mdp} is a tuple, $(S, A, P, R)$, where $S$ is a set of states, $A$ is a set of actions, $P$ is a set of transition probabilities for taking action $a \in A$ at state $s \in S$ and $r\in R(s, a)$ is the reward that qualifies an action $a$ taken at state $s$. A policy, $\pi$, maps $S$ to $A$ and the value $V^{\pi}(s)$ of a state is the expected return for the agent when starting in that state and following the policy. The goal of the agent is to determine an optimal policy, $\pi^*$, that maximizes the expected return.

\begin{equation}
    V^{\pi}(s) = E_{\pi} \Biggl\{
        \sum_{k=0}^{\infty} \gamma^{k}r(s_{k}, \pi(s_{k})) | s_{0} = s
    \Biggr\}
    \label{eqn:value_function}
\end{equation}

In model-based \gls{rl}, $P$ and $R$ are known and an optimal policy, $\pi^*$ can be determined. In most applications, the model dynamics are unknown (model-free \gls{rl}) and the controller must learn to associate optimal actions with states without explicitly determining $P$ or $V^{\pi}(s)$. Tabular Q-Learning \cite{watkins_q-learning_1992} is a popular model-free \gls{rl} algorithm that is based on exploring and exploiting the control space to estimate so-called Q-values. Tabular Q-learning excels in problems with discrete and finite actions, $A$ and states, $S$. However, as $A$ and $S$ increase or become defined over continuous spaces, tabular Q-Learning begins to suffer from the curse of dimensionality. In particular for building control, the curse of dimensionality is significant, considering the potentially large number of sensors measuring various quantities (temperature, humidity, energy consumption, etc.) continuously. This means that the agent has an exponentially increasing number of state-action pairs to explore before it can converge to an optimal solution. Function approximators, e.g., linear regression or artificial neural networks, have been proposed as solutions that allow generalization by directly mapping the state-action pairs to their respective Q-value. There exists different classification of the function approximators for model-free \gls{rl} and we refer the reader to \cite{nagy_ten_2023-1} for their descriptions.

==> latexmkrc <==
add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );

sub makeexternaldocument {
    if (!($root_filename eq $_[0]))
    {
        system( "latexmk -cd -pdf \"$_[0]\"" );
    }
}
